Four-Photon Interference with a High-Efficiency Quantum Dot Source

While two-photon Hong-Ou-Mandel interference visibility has become a standard metric for single-photon sources, many optical quantum technologies require the generation and manipulation of larger photonic states. To date, efficiency limitations have prevented scaling quantum dot-based interference to the coalescence of more than two photons at a single beamsplitter. We overcome this limitation by combining a state-of-the-art quantum dot source with deterministic demultiplexing, enabling the direct observation of quantum interference fringes arising from up to four photons. We measure high mean interference contrasts of $93.0 \pm 0.1~\%$ for two photons, and $84.1 \pm 1.0~\%$ for four photons, with the complex fringe structure fully reproduced by a theoretical model. These results reveal the existence of "deep fringes" whose minima are unaffected by distinguishable photons, rendering the maximum contrast of four-photon interference highly sensitive to multi-photon emission but robust against photon distinguishability. We predict that these phenomena will extend to interference of larger numbers of photons, with relevance across a range of potential optical quantum technologies. A Fisher information analysis demonstrates that interference fringes from our source can exhibit phase sensitivity beyond the standard quantum limit, illustrating potential applications in quantum metrology.

==> latexmkrc <==
$ENV{'TEXINPUTS'}='./tex//:' . $ENV{'TEXINPUTS'};
$ENV{'BSTINPUTS'}='./bst//:' . $ENV{'BSTINPUTS'};

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
